Boosting Flow-based Generative Super-Resolution Models via Learned Prior

Flow-based super-resolution (SR) models have demonstrated astonishing capabilities in generating high-quality images. However, these methods encounter several challenges during image generation, such as grid artifacts, exploding inverses, and suboptimal results due to a fixed sampling temperature. To overcome these issues, this work introduces a conditional learned prior to the inference phase of a flow-based SR model. This prior is a latent code predicted by our proposed latent module conditioned on the low-resolution image, which is then transformed by the flow model into an SR image. Our framework is designed to seamlessly integrate with any contemporary flow-based SR model without modifying its architecture or pre-trained weights. We evaluate the effectiveness of our proposed framework through extensive experiments and ablation analyses. The proposed framework successfully addresses all the inherent issues in flow-based SR models and enhances their performance in various SR scenarios. Our code is available at: https://github.com/liyuantsao/BFSR

==> Equations/z_star.tex <==
\begin{equation}
y = f_\theta^{-1}(z^*; x),
\label{eq:z_to_sr}
\end{equation}

==> Equations/z_to_sr.tex <==
\begin{equation}
    \hat{y} = f_\theta^{-1}(\hat{z}; \cdot),
\label{eq:z_star}
\end{equation}

==> Figures/explode.tex <==
\begin{figure}[t]
  \centering
  \includegraphics[width=1\linewidth]{Figures/Images/explode.pdf}
  \caption{
    When SRFlow integrates with our framework, it effectively prevents generating an exploding inverse. 
  }
  \label{fig:explode}
%   \vspace{-10pt}
\end{figure}

==> Tables/rebuttal_complexity.tex <==
\vspace{-8pt}
\begin{table}[h]
\renewcommand{\arraystretch}{1.2}
\centering
\tiny
\resizebox{0.75\columnwidth}{!}{%
    \begin{tabular}{l|c|c}
        \hline
         & RRDB-LINF & Latent Module  \\
        \hline
        Time (s) & 0.4975 & 0.0033 \\
        \hline
    \end{tabular}
}
\vspace{-8pt}
\caption{Forward pass time of our flow model and the latent module. The average inference time for 4$\times$ SR on the DIV2K validation set is reported.}
% \caption{The average 4$\times$ SR running time on DIV2K validation set, evaluated on an NVIDIA Geforce RTX 3090.}
\label{tab:complexity}
\end{table}
